Loss Minimization of Traction Systems in Battery Electric Vehicles Using Variable DC-link Voltage Technique -- Experimental Study

A novel variable dc-link voltage technique is proposed to reduce the traction losses for electrical drive applications. A 100-unit cascaded multilevel converter is developed to generate the variable dc-link voltage. Experimental measurement shows that the machine additional losses and IGBT-inverter losses are reduced substantially. The system efficiency enhancement is at least 2%.

==> chapters/00_header.tex <==
%For printing a title, please use \EPEtitle
\EPEtitle{Loss Minimization of Traction Systems in Battery Electric Vehicle Using Variable DC-link Voltage Technique}

%\author{
%The author's name\\
%THE AUTHOR'S COMPANY\\
%Address\\
%City, Country\\
%Phone: +xx (x) xxx-xxxx\\
%Fax: +xx (x) xxx-xxxx\\
%Email: Author.Name@Company.com\\
%URL: http://www.company.com}
\date{}										%print no date

\maketitle


\section*{Keywords}
%Please use \EPEkeyword to include your keywords to ensure correct format
 \EPEkeyword{Loss minimization}, \EPEkeyword{Modular multilevel converter}, \EPEkeyword{Variable dc-link voltage}, \EPEkeyword{Electrical drives}, \EPEkeyword{Battery balancing}. 
